Quantum Reservoir Computing and Risk Bounds

We propose a way to bound the generalisation errors of several classes of quantum reservoirs using the Rademacher complexity. We give specific, parameter-dependent bounds for two particular quantum reservoir classes. We analyse how the generalisation bounds scale with growing numbers of qubits. Applying our results to classes with polynomial readout functions, we find that the risk bounds converge in the number of training samples. The explicit dependence on the quantum reservoir and readout parameters in our bounds can be used to control the generalisation error to a certain extent. It should be noted that the bounds scale exponentially with the number of qubits n. The upper bounds on the Rademacher complexity can be applied to other reservoir classes that fulfill a few hypotheses on the quantum dynamics and the readout function.

==> proof_prop_l_omega_poly.tex <==

For ease of notation, we write $x_{r_{i_j}} = \text{tr}\left[ \sigma_Z^{(i_j)} \rho \right]^{r_{i_j}}$.

We will show that all functions in $\Tilde{\mathcal{F}}_{n, R_{\max}, C_{\max}}^{\text{poly}} $ are Lipschitz-continuous w.r.t. the parameters $\omega = (C, \pmb w)$ and thus, 
    For any fixed $\rho \in \Bplus \cup 0 \rightarrow \mathbb{R}$, for all $(C, \pmb w), (C', \tilde{\pmb w}) \in \Omega_{\text{poly}}$, we have
    \begin{align}
        & \left\vert h_{C, \pmb w} (\rho) - h_{C', \tilde{\pmb w}} (\rho) \right\vert \\
        &= \left\vert C - C' + \sum_{d=1}^{R_{\text{max}}}\sum_{i_1=1}^n\sum_{i_2=i_1+1}^n \cdots \sum_{i_n = i_{n-1}+1}^n \sum_{r_{i_1}+\cdots + r_{i_n}=d} \left( w_{i_1,\ldots,i_n}^{r_{i_1},\ldots,r_{i_n}} - \tilde{w}_{i_1,\ldots,i_n}^{r_{i_1},\ldots,r_{i_n}}  \right) x_{r_{i_1}} \cdots x_{r_{i_n}} \right\vert \\
        & \leq \left\vert C - C' \right\vert +  \sum_{d=1}^{R_{\text{max}}}\sum_{i_1=1}^n\sum_{i_2=i_1+1}^n \cdots \sum_{i_n = i_{n-1}+1}^n \sum_{r_{i_1}+\cdots + r_{i_n}=d} \left\vert\left( w_{i_1,\ldots,i_n}^{r_{i_1},\ldots,r_{i_n}} - \tilde{w}_{i_1,\ldots,i_n}^{r_{i_1},\ldots,r_{i_n}}  \right)\right\vert \left\vert x_{r_{i_1}} \cdots x_{r_{i_n}} \right\vert \\
        & \leq \left\Vert (C, \pmb w) - (C', \tilde{\pmb w}) \right\Vert_1 \leq  \sqrt{\mathcal{N}_{\text{poly}} + 1 } \left\Vert (C, \pmb w) - (C', \tilde{\pmb w}) \right\Vert_2
    \end{align}
    where we have used the fact that the traces of the density matrices are all between $-1$ and $1$ in the second to last inequality, and we have bounded the one norm via the two norm.


